Virtual Array for Dual Function MIMO Radar Communication Systems using OTFS Waveforms

A MIMO dual-function radar communication (DFRC) system transmitting orthogonal time frequency space (OTFS) waveforms is considered. A key advantage of MIMO radar is its ability to create a virtual array, achieving higher sensing resolution than the physical receive array. In this paper, we propose a novel approach to construct a virtual array for the system under consideration. The transmit antennas can use the Doppler-delay (DD) domain bins in a shared fashion. A number of Time-Frequency (TF) bins, referred to as private bins, are exclusively assigned to specific transmit antennas. The TF signals received on the private bins are orthogonal and thus can be used to synthesize a virtual array, which, combined with coarse knowledge of radar parameters (i.e., angle, range, and velocity), enables high-resolution estimation of those parameters. The introduction of $N_p$ private bins necessitates a reduction in DD domain symbols, thereby reducing the data rate of each transmit antenna by $N_p-1$. However, even a small number of private bins is sufficient to achieve significant sensing gains with minimal communication rate loss.

==> Format.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Packages to Load
%% Text and Math Environment Packages
\RequirePackage{csquotes} %Package to Facilities Quotations
% \RequirePackage[backend=biber, style=numeric, sorting=none]{biblatex}
\RequirePackage[english]{babel} %Multilingual Support Must Load the First
% \RequirePackage[utf8]{inputenc} %utf8 Support. Preloaded in Distribution
\RequirePackage[T1]{fontenc} %Better Font Encoding for T1 Type Font
\RequirePackage[shortlabels, inline]{enumitem} %Conflict with Beamer
\RequirePackage[svgnames]{xcolor} %Beamer Has This by Default
\RequirePackage[most]{tcolorbox} %Customized Box. Must Load after xcolor
\RequirePackage{mathtools} %Customize Math Symbols and Theorems
\RequirePackage{amsthm, thmtools, thm-restate} %Better Theorems
% \RiquirePackage{amsmath} %Loaded by mathtools
% \RequirePackage{amssymb} %Conflict with Fonts
\RequirePackage{Fonts} %Must Load after tcolorbox and amsthm
% \let\openbox\undefined %Fix Some Font Issues
\RequirePackage{bm} %Boldface Math, Load after Other Math Font Packages
\RequirePackage{mleftright} %Fixes Some Math Spacing Issues
\RequirePackage{microtype} %Better Font Spacing

%% Table Packages
\RequirePackage{tabularx} %Including Tabular with More Space Option
\RequirePackage{colortbl} %Package to Use Color in Tables
\RequirePackage{multirow} %Package to Use Multirow in Tables
\RequirePackage{multicol} %Package to Use Multicols
\RequirePackage{array} %Math and More Spacing Support in Tables

%% Graphics Packages
\RequirePackage{epstopdf} %Package to Convert eps to pdf in pdfLatex
\RequirePackage{transparent} %Transparent Images
\RequirePackage{graphicx} %Graphics Backend with key-value Arguments
\RequirePackage[export]{adjustbox} %More Arguments for includegraphics
\RequirePackage{subcaption} %Package to Use Subfigure

%% Code Packages
% \RequirePackage{listings} %Loaded by tcolorbox and also no need of minted.
\RequirePackage{algorithm} %Package to Insert Algorithm
\RequirePackage{algpseudocode} %Package to Insert Algorithm

%% Other Packages
\RequirePackage{xspace} %Package to Add Space after Macros
% \RequirePackage{calc} %Package of Calculation in Latex
% \RequirePackage{rotating} %Package to Rotate Objects
% \RequirePackage{pgf, tikz} %Package to Draw Figures.
% \RequirePackage{keyval}
\RequirePackage{orcidlink}
% \RequirePackage{hyperref} %Beamer Has This by Default.
% \RequirePackage{cleveref} %Must Load after others. Conflict with Beamer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
